Intra-class variation reduction of speaker representation in disentanglement framework

In this paper, we propose an effective training strategy to ex-tract robust speaker representations from a speech signal. Oneof the key challenges in speaker recognition tasks is to learnlatent representations or embeddings containing solely speakercharacteristic information in order to be robust in terms of intra-speaker variations. By modifying the network architecture togenerate both speaker-related and speaker-unrelated representa-tions, we exploit a learning criterion which minimizes the mu-tual information between these disentangled embeddings. Wealso introduce an identity change loss criterion which utilizes areconstruction error to different utterances spoken by the samespeaker. Since the proposed criteria reduce the variation ofspeaker characteristics caused by changes in background envi-ronment or spoken content, the resulting embeddings of eachspeaker become more consistent. The effectiveness of the pro-posed method is demonstrated through two tasks; disentangle-ment performance, and improvement of speaker recognition ac-curacy compared to the baseline model on a benchmark dataset,VoxCeleb1. Ablation studies also show the impact of each cri-terion on overall performance.

==> ______.tex <==
\section{Discussion}

\begin{comment}
\subsection{Training strategy}
\noindent The training process consists of three phases.

\noindent \textbf{Phase I.}
% \vspace{5pt}
All parameters are initialized by the Xavier method~\cite{glorot2010understanding}.
In this phase, the speaker encoder $E_{id}$ is trained using the speaker loss $L_s$.
A learning rate is set to 0.001.
%Speaker encoder should be trained in prior to other stages since  

\noindent \textbf{Phase II.}
% Kang: 흐름 다시 정리할 것.
%\vspace{5pt}
When we train the whole networks using all criteria simultaneously, the network does not converge well.
Thus, it is necessary to limit the embedding space to be placed in the appropriate vector space such that it can be understood well by the network.
Before training the other network, we fix the speaker encoder after phase I.
% Kang: 아래 문장 다시 정확하게 서술 필요.
Then, we train the residual encoder $E_{res}$, decoder $G$, MINE network $T$ and discriminator $D_d,D_c$ with disentanglement loss, reconstruction loss, id change loss and discriminator loss.

\noindent \textbf{Phase III.}
Finally, we train the whole network with an end-to-end manner until converged.
Since all of the networks are already trained once, phase III. is considered as a kind of fine tuning process.
We set the learning rate to 1e-4 for the training.
\end{comment}




 This way, the gradient computed within the encoder not only depends on the supervised
loss but also on the unsupervised objective. The latter approach
turned out to be very effective, since the unsupervised gradient
acts as a powerful regularizer

% 현재 discriminator 제외한 실험 중이서 해당 내용 빼고 수정하였습니다.
%The reconstructed spectrum, $\hat{S}_{mel}$, is used as an input of the multi-task discriminator that consists of a class discriminator, $D_c$ and a domain discriminator, $D_d$.
%The class discriminator determines the identity of input, and the domain discriminator distinguishes whether the input mel-spectrum is real or fake.

\begin{comment}
\noindent\textbf{Discriminator loss.}
We use multi-task discriminators, $D_d$ and $D_c$. 
The $D_d$ helps the generator $D_r$ to reconstruct more realistic spectrum, and the class discriminator $D_c$ forces the synthesized output to have speaker characteristics.
The loss function of each discriminator, $L_d$ and $L_c$ is defined as follows:
\begin{equation}
\begin{split}
    L_d=&min~max[\sum logD_d(S) \\
        & \qquad {} + \sum log(1-D_d(D_r(f_{spk},f_{res})))],
\end{split}
\end{equation}
\begin{equation}
  L_c= -\sum_{c=1}^{C}\sum_{k=1}^{K}q_c^klogD_c(S),
\end{equation}
where $S$ is a mel-spectrum fed to the discriminator, $C$ is the number of speaker, and $k$ is the number of samples.
\vspace{5pt}
\end{comment}
\begin{comment}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{IC_loss_ver2.png}
  \caption{Description of identity interchange loss.}
  \label{fig:loss}
\end{figure}

\end{comment}



%experiment내용
%%%%comment out
\begin{comment}
Table \ref{table:2} shows equal error rates (EERs) obtained by ablation studies, which provides the effectiveness of loss functions used in proposed model.
From the experiment 1~3, we confirm that minimizing the mutual information between speaker and residual embeddings is effective to disentangle the speaker information from input speech compared to the adversarial training method which is used in our baseline.
Unlike the disentanglement method via adversarial training, which is applied to the encoders independently, mutual information is calculated between speaker and residual embedding simultaneously, resulting in more powerful disentanglement results.
The experiment 4 demonstrates the proposed identity change loss is effective to speaker recognition.
Idnetity change loss utilzes speaker embeddings extracted from different utterances to regenerate input speech, which helps to extract a constant speaker embedding, or common identity, in utterance with different linguistic information.
Fig.~\ref{fig:fig} illustrates t-SNE plots~\cite{maaten2008visualizing} to visualize the effectiveness of the proposed method.
Fig.~\ref{fig:sub-first},\ref{fig:sub-second} are the plots of embedding extracted from the speaker and residual encoder, $E_{spk}$, $E_{res}$, trained by the mutual information criterion.
The features generated by the speaker encoder are well-clustered but those by the residual encoder are randomly distributed in the low-dimensional feature space. 
It demonstrate the mutual information effectively separate the speaker information and residual embedding and embeds into each embedding, repectively.
Fig.~\ref{fig:sub-first} and \ref{fig:sub-second} illustrate the plot of speaker embeddings extracted from the baseline model and the ones from the proposed model with the MI and identity change loss.
As shown in these figures, the clusters obtained by the proposed method show clearer boundaries between identities and smaller distances to the same identities.
\end{comment}


% \begin{comment}
% \begin{equation}
%   L_{mi} = \mathbb{E}_{p}[T_\theta(P)]-log(\mathbb{E}_{n}[e^{T_\theta(N)}]).
%  \label{mi_loss}
% \end{equation}
% We use mutual information as a criterion to disentangle speaker embedding $f_{spk}$ and residual embedding $f_{res}$ according to the \emph{MINE} algorithm proposed in ~\cite{belghazi2018mine}.
% \begin{equation}
%   L_{mi}=\hat{I}_T(f_{spk},f_{res}),
% \end{equation}
% where $\hat{I}_T(a, b)$ denotes mutual information between embedding $a$ and $b$.
% % Kang (5/14) 아래 문장 이해 안됨. 다시 서술할 것.
% For applying \emph{MINE}, we draws samples from the joint and product of marginals distribution, respectively.
% To maximize the discrepancy between speaker and residual embedding, we draw positive samples $P=(f_{A,spk},f_{A',spk})$, negative samples $N=(f_{A,spk},f_{A,res})$ and vice versa from same utterance as shown in Fig.~\ref{fig:sub-mine}.
% \begin{equation}
%   L_{mi} = \mathbb{E}_{p}[T_\theta(P)]-log(\mathbb{E}_{n}[e^{T_\theta(N)}]).
%  \label{mi_loss}
% \end{equation}
% % Kang (5/14) 아래 두 문장 위치 흐름상 적합하지 않음. 앞 부분, 예를 들면 related works 마지막 부분, 으로 옮겨서 다시 설명할 것.
% %Although the adversarial training tries not to include speaker information into the residual embedding, it does not consider the relation between the embeddings directly.
% A minimization of mutual information between the speaker and residual embeddings is used so that two embeddings do not share informatively common characteristics.

% While the adversarial classifier is trained to classify the speaker identity correctly, the residual encoder is trained to fool the classifier, such that it eliminates the speaker information from residual embedding.
% We introduce mutual information loss for separating into speaker-related and unrelated embedding.
% Mutual information has an advantage in decoupling the information by considering the relation of speaker and residual embedding at once, unlike the adversarial loss which is used in baseline.

% Our \emph{MINE} system, depicted in Fig.~\ref{fig:sub-mine}, is trained to minimize the mutual information between speaker embedding $f_{spk}$ and residual embedding $f_{res}$ for disentangled features.
% To measure the MI, we draws the samples from joint distribution and product of marginals distributions, respectively.
% we set the samples from joint distribution as $(f_{A,spk},f_{A',spk})$ and from product of marginals as $(f_{A,spk},f_{A,res})$ as shown in Fig.~\ref{fig:sub-mine}.
% Under these setting, the mutual information loss is described as:
% \begin{equation}
%   \label{mi_loss}
%  \begin{split}
%       L_{MI} = &\mathbb{E}[T_\theta(f_{A,spk},f_{A',spk})]- \\
%               &log(\mathbb{E}[e^{T_\theta(f_{A,spk},f_{A,res})}]).
%  \end{split}
% \end{equation}
% A minimization of mutual information between the speaker and residual embeddings is used so that two embeddings do not share informatively common characteristics.
% \end{comment}

\begin{comment}
To apply the identity change loss, it needs a pair of speech spoken by a same speaker.
At first, we extract both speaker and residual embeddings using the speaker and residual encoder.
To reduce the difference in intra-cluster, the speaker embedding is replaced with a mean of all the speaker embedding from the same speaker and they are fed to the decoder.
Finally, using the reconstructed mel-spectrum $\hat{S}_{A}=D_r(f_{mean,spk}, f_{A,res})$ and $\hat{S}_{B}=D_r(f_{mean,spk}, f_{B,res})$, the reconstruction loss is calculated for training.
\begin{equation}
 \begin{split}
     L_{ch}=&L_r(\hat{S}_{A}) + L_r(\hat{S}_{B}).
 \end{split}
\end{equation}
Although the speaker embeddings are replaced, the generated mel-spectrum should be the same as the original one because the pair has the same speaker identity.
This identity chage process encourages the speaker encoder $E_{spk}$ to focus on common information and makes speaker embedding robust to intra-variations.
\end{comment}

\begin{figure*}[t]
\begin{subfigure}{.19\textwidth}
  \centering
  \includegraphics[width=\linewidth]{base_loss.png}  
  \caption{Baseline loss}
  \label{fig:baseloss}
\end{subfigure}

\rulesep

\begin{subfigure}{.418\textwidth}
  \centering
  \includegraphics[width=\linewidth]{id_change_loss.png}  
  \caption{Identity change loss}
  \label{fig:idloss}
\end{subfigure}

\rulesep

\begin{subfigure}{.342\textwidth}
  \centering
  \includegraphics[width=\linewidth]{mine_loss.png}  
  \caption{Mutual information loss}
  \label{mineloss}
\end{subfigure}

\caption{Overview of proposed training criteria. {\normalfont (a)} Training criteria based on ~\cite{Tai2020SEFALDRAS}: spekeaker loss, disentanglement loss and reconstruction loss. 
{\normalfont (b)} Identity change loss: switch the spekaer embedding to mean of those.
{\normalfont (c)} Mutual information loss: estimate the mutual information by MINE} 
 
\label{fig:overall}
\end{figure*}
